Measurement-Based Quantum Approximate Optimization

Parameterized quantum circuits are attractive candidates for potential quantum advantage in the near term and beyond. At the same time, as quantum computing hardware not only continues to improve but also begins to incorporate new features such as mid-circuit measurement and adaptive control, opportunities arise for innovative algorithmic paradigms. In this work we focus on measurement-based quantum computing protocols for approximate optimization, in particular related to quantum alternating operator ans\"atze (QAOA), a popular quantum circuit model approach to combinatorial optimization. For the construction and analysis of our measurement-based protocols we demonstrate that diagrammatic approaches, specifically ZX-calculus and its extensions, are effective for adapting such algorithms to the measurement-based setting. In particular we derive measurement patterns for applying QAOA to the broad and important class of QUBO problems. We further outline how for constrained optimization, hard problem constraints may be directly incorporated into our protocol to guarantee the feasibility of the solution found and avoid the need for dealing with penalties. Finally we discuss the resource requirements and tradeoffs of our approach to that of more traditional quantum circuits.

==> makefile <==
LATEXCMDS := -pdf \
			 -pdflatex \
			 -bibtex \
			 --outdir=build \
			 -bibfudge \
			 -shell-escape

all: tex

tex: main.tex tikz/*.tex
	mkdir -p build
	mkdir -p build/externalized
	latexmk $(LATEXCMDS) main.tex 

keeprunning: 
	mkdir -p build
	mkdir -p build/externalized
	latexmk $(LATEXCMDS) -pvc main.tex 

clean:
	rm build/*

